Vid2Avatar-Pro: Authentic Avatar from Videos in the Wild via Universal Prior

We present Vid2Avatar-Pro, a method to create photorealistic and animatable 3D human avatars from monocular in-the-wild videos. Building a high-quality avatar that supports animation with diverse poses from a monocular video is challenging because the observation of pose diversity and view points is inherently limited. The lack of pose variations typically leads to poor generalization to novel poses, and avatars can easily overfit to limited input view points, producing artifacts and distortions from other views. In this work, we address these limitations by leveraging a universal prior model (UPM) learned from a large corpus of multi-view clothed human performance capture data. We build our representation on top of expressive 3D Gaussians with canonical front and back maps shared across identities. Once the UPM is learned to accurately reproduce the large-scale multi-view human images, we fine-tune the model with an in-the-wild video via inverse rendering to obtain a personalized photorealistic human avatar that can be faithfully animated to novel human motions and rendered from novel views. The experiments show that our approach based on the learned universal prior sets a new state-of-the-art in monocular avatar reconstruction by substantially outperforming existing approaches relying only on heuristic regularization or a shape prior of minimally clothed bodies (e.g., SMPL) on publicly available datasets.

==> sec/03_data.tex <==
% \section{Preliminary}
% \paragraph{Training Data Acquisition.}
% \label{sec:corpus}
% We use a multi-view system similar to \cite{bagautdinov2021driving} to capture dynamic human performance, where we obtain calibrated and synchronized multi-view images at a resolution of 4096$\times$2668 pixels through the use of 200 cameras. 
% %
% Participants are instructed to perform casual human motions for approximately 10,000 frames per person on average. In total, 1000 participants are recorded for model training.
